DialGuide: Aligning Dialogue Model Behavior with Developer Guidelines

Dialogue models are able to generate coherent and fluent responses, but they can still be challenging to control and may produce non-engaging, unsafe results. This unpredictability diminishes user trust and can hinder the use of the models in the real world. To address this, we introduce DialGuide, a novel framework for controlling dialogue model behavior using natural language rules, or guidelines. These guidelines provide information about the context they are applicable to and what should be included in the response, allowing the models to generate responses that are more closely aligned with the developer's expectations and intent. We evaluate DialGuide on three tasks in open-domain dialogue response generation: guideline selection, response generation, and response entailment verification. Our dataset contains 10,737 positive and 15,467 negative dialogue context-response-guideline triplets across two domains - chit-chat and safety. We provide baseline models for the tasks and benchmark their performance. We also demonstrate that DialGuide is effective in the dialogue safety domain, producing safe and engaging responses that follow developer guidelines.

==> guideline/04-experimetsv1.tex <==



\begin{table*}[ht]
\small
\centering
\begin{tabular}{lrrrrrrr}
\toprule
Model & \multicolumn{1}{l}{map@1} & \multicolumn{1}{l}{map@3} &
\multicolumn{1}{l}{map@10} & \multicolumn{1}{l}{mrr} & \multicolumn{1}{l}{ndcg@3} & \multicolumn{1}{l}{recall@3} & \multicolumn{1}{l}{recall@5} \\
\hline
BM25 & 12.9 & 23.4 & 46.4 & 52.7 & 25.0 & 30.8 & 45.6 \\
% DPR (synthetic) & 21.8 & 39 & 63.4 & 70.5 & 55.1 & 44.4 & 66.9 \\
% DPR (synthetic+adv) & 28.8 & 53.4 & 75.1 & 83.4 & 71.6 & 60.4 & 80.5 \\
DPR (silver) & 29.8 & 52.6 & 73.9 & 83.4 & 70.0 & 58.3 & 77.1 \\
DPR (silver+adv) & 31.7 & 59.4 & 78.9 & 86.9 & 76.9 & 66.0 & 83.2 \\
Rerank-deberta (silver) & 30.2 & 56.6 & 76.9 & 83.9 & 73.6 & 63.5 & 83.5 \\
Rerank-deberta (ann)& 34.6 & {71.4} & 88.2 & 91.1 & 87.7 & 78.0 & 93.9 \\
Rerank-deberta (silver+ann) & \textbf{37.5} & \textbf{73.7} & \textbf{90.7} & \textbf{94.1} & \textbf{89.6} & \textbf{78.1} & \textbf{94.5} \\
\bottomrule
\end{tabular}
\caption{Guideline retrieval results. Re-ranking models performs better than DPR. The model trained on the combined set of silver and human annotated guidelines performs the best.}
\label{tab:retrievalresults}
\vspace{-2mm}
\end{table*}

% \begin{table*}[t]
% \small
% \centering

% \begin{tabular}{lrrrrrrrr}
% \toprule

%  & \multicolumn{4}{c}{Normal test set} & \multicolumn{4}{c}{Adversarial test set} \\
%  \hline
% Model & \multicolumn{1}{l}{F1 (yes)} & \multicolumn{1}{l}{F1 (no)} & \multicolumn{1}{l}{Macro F1} & \multicolumn{1}{l}{Acc} & \multicolumn{1}{l}{F1 (yes)} & \multicolumn{1}{l}{F1 (no)} & \multicolumn{1}{l}{Macro F1} & \multicolumn{1}{l}{Acc} \\
% \hline
% Semantic & 0.42 & 0.72 & 0.58 & 0.64 & 0.36 & 0.73 & 0.54 & 0.62 \\
% DNLI & 0.38 & 0.64 & 0.51 & 0.53 & 0.36 & 0.71 & 0.54 & 0.61 \\
% DialBart0 & 0.68 & 0.26 & 0.56 & 0.56 & 0.55 & 0.25 & 0.4 & 0.44 \\
% % DialBart tuned & 0.79 & 0.8 & 0.79 & 0.79 & 0.7 & 0.81 & 0.76 & 0.76 \\
% DialBart-BST & 0.84 & 0.81 & 0.83 & 0.83 & 0.73 & 0.77 & 0.76 & 0.75 \\
% DialBart-BST-Adv & 0.84 & 0.84 & 0.84 & 0.84 & \textbf{0.79} & \textbf{0.86} & \textbf{0.83} & \textbf{0.83} \\
% %semantic, dnli, dialfact, noguidelinetestonly, dialt0, dialt0tuned, dialt0tunedadv
% \bottomrule
% \end{tabular}
% \caption{Guideline-based response selection results. The model trained on the annotated dataset performs well. Training on the adversarial set improves performance on the adversarial test set without reducing performance on the normal test set.}
% \label{tab:selectionresults}
% \vspace{-2mm}
% \end{table*}



\begin{table*}[t]
\small
\centering

% \begin{tabular}{lrrrrrrrr}
\begin{tabular}{lcccccccc}
\toprule

 & \multicolumn{4}{c}{Normal test set} & \multicolumn{4}{c}{Adversarial test set} \\
 \cmidrule(lr){2-5} \cmidrule(lr){6-9}
%  \hline
Model & \multicolumn{1}{c}{F1 (yes)} & \multicolumn{1}{c}{F1 (no)} & \multicolumn{1}{c}{Macro F1} & \multicolumn{1}{c}{Acc} & \multicolumn{1}{c}{F1 (yes)} & \multicolumn{1}{c}{F1 (no)} & \multicolumn{1}{c}{Macro F1} & \multicolumn{1}{c}{Acc} \\
\hline
% \cmidrule(lr){1-9}
% Semantic & 0.42 & 0.72 & 0.58 & 0.64 & 0.36 & 0.73 & 0.54 & 0.62 \\
% Semantic & 51.9 & 74.6 & 63.3 & 66.8 & 43.4 & 72.0 & 57.7 & 62.6 \\ #nocontext
% Token overlap & 47.4 & 63.8 & 55.6 & 57.1 & 40.5 & 63.3 & 51.9 & 54.6 \\
% DNLI & 38.0 & 64.2 & 51.5 & 53.2 & 36.1 & 67.8 & 54.2 & 57.4 \\
% DialT0-Zeroshot & 59.5 & 39.5 & 42.1 & 49.0 & 50.7 & 29.0 & 35.6 & 41.8\\ % below is when context is used, performance drops
% % Roberta-Large & 14.3 & 77.4 & 45.9 & 64.2 & 14.1 & 82.4 & 48.2 & 70.8 \\
% Roberta-Large & 80.8 & 89.1 & 85.9 & 86.1 & 73.8 & 87.8 & 83.5 & 83.3 \\
% BSTGuide-T5XL & 87.2 & 92.2 & 90.3 & 90.3 & 80.8 & 90.6 & 87.6 & 87.4 \\
% BSTGuide-NoAdv & 87.4 & 92.6 & 90.6 & 90.7 & 79.0 & 89.8 & 86.4 & 86.2 \\
% BSTGuide & \textbf{87.7} & \textbf{92.6} & \textbf{90.8} & 90.8 & \textbf{83.0} & \textbf{92.0} & \textbf{89.3} & \textbf{89.2} \\

Token-overlap & 47.4 & 63.8 & 55.6 & 57.1 & 40.5 & 63.3 & 51.9 & 54.6 \\
DNLI & 38.0 & 64.2 & 51.5 & 53.2 & 36.1 & 67.8 & 54.2 & 57.4 \\
DialT0-Zeroshot & 59.5 & 39.5 & 30.3 & 49.0 & 50.7 & 29.0 & 26.6 & 41.8\\ % below is when context is used, performance drops
% Roberta-Large & 14.3 & 77.4 & 45.9 & 64.2 & 14.1 & 82.4 & 48.2 & 70.8 \\
Roberta-Large & 80.8 & 89.1 & 84.9 & 86.1 & 73.8 & 87.8 & 81.5 & 83.3 \\
BSTGuide-T5XL & 87.2 & 92.2 & 89.7 & 90.3 & 80.8 & 90.6 & 85.7 & 87.4 \\
BSTGuide-NoAdv & 87.4 & \textbf{92.6} & 90.0 & 90.7 & 79.0 & 89.8 & 84.3 & 86.2 \\
BSTGuide & \textbf{87.7} & \textbf{92.6} & \textbf{90.2} & \textbf{90.8} & \textbf{83.0} & \textbf{92.0} & \textbf{87.5} & \textbf{89.2} \\

%semantic, dnli, dialfact, noguidelinetestonly, bert, dialt0, t5tuned, dialt0tuned, dialt0tunedadv
\bottomrule
\end{tabular}
\caption{Guideline-based response entailment verification results. The model trained on the annotated dataset performs well. Training on the adversarial set improves performance on the adversarial test set without reducing performance on the normal test set.}
\label{tab:selectionresults}
\vspace{-2mm}
\end{table*}




\section{Experiments and Results}
\label{sec:experiments}
In this section we discuss the experimental setup and results for the three tasks --- 1) Guideline retrieval, 2) Response selection, and 3) Response entailment verification.

% \subsection{Model Details}


% \subsection{Training Details}


\subsection{Guideline Retrieval}
\label{sec:guidelineretrieval}
\subsubsection{Setup and Baselines}
This task consists of retrieving the guidelines most relevant to a context.
For a context $C$, the guideline set $G_c \owns (g_1,g_2,..g_k)$ is composed of 10 guidelines and binary human annotations of whether a guideline condition is relevant to the context. The candidate set contains the gold human-written guideline and hence consists of at least one relevant guideline.
For this task, we only use the condition part of the guideline and ignore the action part. We experiment on the train, dev and test sets of \dataname-\textsc{BST}, with 2798, 1004 and 1011 context respectively and 10 candidate guidelines annotated per context. We use standard retrieval metrics such as Recall and MRR.

For training data, we use the following guideline-context pairs discussed in Section \ref{sec:task} -- a) Human annotated data: Consists of human annotations collected in the guideline annotation task. A positive pair consists of a context and a guideline annotated as relevant to the context. An easy negative pair consists of a context and a randomly selected guideline.
A hard negative pair consists of a guideline annotated as irrelevant to the context following \cite{karpukhin-etal-2020-dense};
b) Silver data: The synthetic guidelines set $G_{BST}$ created using $M_g$ consists of 33k guidelines-context pairs. We do not have human annotations for these guidelines. A positive pair consists of a context and a guideline generated for the context. A negative pair consists of a context and a randomly selected guideline.

We experiment with the following methods -
\begin{itemize}[noitemsep,nolistsep,leftmargin=*]
% \begin{itemize}
\item {BM25}: Measures overlap between the guideline and the context. 
\item DPR~\cite{karpukhin-etal-2020-dense} (silver): The base DPR model is a bert-base bi-encoder model trained on the Natural Questions dataset. We fine-tune it on silver guideline-context pairs. 
\item DPR (silver+ann): DPR model fine-tuned on both silver and human annotated pairs.
\item Rerank-deberta (silver): Deberta~\cite{he2020deberta} based classification model trained using the silver guideline-context pairs.
\item Rerank-deberta (ann): Deberta model trained only on human annotated guidelines.
\item Rerank-deberta (silver+ann): Deberta model trained on both silver and human annotated pairs.
\end{itemize}



% \subsubsection{Training Details}
For training the DPR models, we use a batch size of 16 for 50 epochs.
For the Deberta models, we fine-tune the Deberta-base model with a batch size of 60 across 8 GPUs.

\subsubsection{Results}
We show the guideline retrieval results in Table~\ref{tab:retrievalresults}. We observe that the BM25 model performs poorly, which shows that simple word-based prediction does not work on this task. Although DPR and Deberta models trained using human annotated data perform the best, models trained on silver data also show reasonable performance. This shows the potential of bootstrapping a retriever for a new domain using silver data from synthetic guidelines. 
Overall the Deberta model performs better than DPR and BM25 baselines.
The Deberta model trained on the combination of human annotated and silver data performs better than the model trained on the smaller set of human guidelines, implying that data augmentation benefits this task. 
Our best model has a recall@3 of around 78\%, making it suitable for practical purposes.
% For practical purposes, these baselines can be combined by first retrieving  a larger set of guidelines using BM25 + DPR for faster inference, and then reranking them using the Deberta models.


% \section{Experimental setup}

% \subsection{Dataset}
% The dataset statistics are shown in Table~\ref{tab:bststats} and ~\ref{tab:safetystats}. We show stats for all the three tasks.







\subsection{Response Entailment Verification}
\subsubsection{Setup and Baselines}
This is a binary classification task to predict whether a response follows the provided guideline and is coherent to the context.
We experiment on the train, dev and test sets of \dataname-\textsc{BST} with 14689, 4406 and 4962 context-response pairs (the distribution shown in Table~\ref{tab:bststats}). 
Two settings are used: 1) Normal, where we only use the Positive and Negative  instances, and 2) Adversarial, which additionally consists of adversarial negative responses (described in Section~\ref{sec:task}).  We report the F1 scores per class, macro F1 and accuracy.
We explore the following models and baselines:
\begin{itemize}[noitemsep,nolistsep,leftmargin=*]
% \begin{itemize}
\item {Token-overlap}: Measures token level overlap between the guideline and the response after stop-word removal. A threshold (tuned using the dev set) is used for classification.
\item {DNLI}~\cite{welleck-etal-2019-dialogue}: A model trained on the Dialogue NLI task.
\item{Roberta-Large}: A Deberta~\cite{liu2019roberta} based classification model.
\item {DialT0-Zeroshot}:
% Bart~\cite{lewis-etal-2020-bart} and T5~\cite{JMLRt5}
 A multi-task and instruction based model pre-trained on multiple dialogue tasks from Instructdial~\cite{gupta2022improving} and tested on this task in a zero-shot setting. This is based on T5~\cite{JMLRt5} architecture and contains 3 billion parameters.
\item {BSTGuide-T5XL}: A T5-XL model fine-tuned on positive and negative as well as adversarial negative examples from the train set.
\item {BSTGuide-NoAdv}: A DialT0 model fine-tuned on the positive and negative  examples from the train set.
% \item {DialT5-BST}: DialT0 model fine-tuned on positive and negative examples from train set.
\item {BSTGuide}: A DialT0 model fine-tuned on the positive and negative as well as adversarial negative  examples from the train set.
\end{itemize}

% \subsubsection{Training Details}
The DNLI model is a \greytext{Bert-type} model that is trained on the Dialogue NLI dataset. 
% We use the \greytext{base} version of the Deberta model.
% DialBart-BST (400M parameters) and DialT5-BST (3B parameters) are Instructdial pretrained models fine-tuned on conversations and guidelines from \dataname-\textsc{BST}. 
For all Dial* baselines, the guideline is concatenated to the dialogue context and the response candidate. 
% \subsubsection{Setup and Baselines}



\subsubsection{Results}
The results are presented in Table~\ref{tab:selectionresults}. The Token-overlap and DNLI models perform poorly on the task, indicating that the task needs models with capabilities beyond the token level overlap for semantic similarity measures. The DialT0 multi-task pretrained models also struggle on this task in the zero-shot setting. 
Our model {BSTGuide}  shows the best performance, achieving
{90.8}\% 
accuracy and {90.2} macro F1 score on the Normal test set.
We see a performance drop when testing on the Adversarial test set ---({89.2}\%  accuracy and {87.5} macro F1), verifying that our Adversarial test set contains difficult test cases. However, the performance drop is lower than that of the BSTGuide-NoAdv model that has been fine-tuned on our training set excluding adversarial examples, indicating that training on a few adversarial examples makes the model more robust.
Finally, the {BSTGuide} (base DialT0 model tuned on \dataname) outperforms  the BSTGuide-T5XL (base T5 model tuned on \dataname), which shows that the DialT0 model pretrained on multiple dialogue tasks (such as commonsense QA and NLI tasks) serves as a better model for this task.






\begin{table*}[t]
\small
\centering
\addtolength{\tabcolsep}{-1pt}
% \setlength\tabcolsep{3pt}
 \begin{tabular}{lrrrrrrrrr}
%\begin{tabularx}{\linewidth}{l*{9}}
\toprule
Model &
  \multicolumn{1}{c}{Bleu-2} &
  \multicolumn{1}{c}{Bleu-4} &
  \multicolumn{1}{c}{RougeL} &
  \multicolumn{1}{c}{Gd-Bleu-2 $\downarrow$} &
  \multicolumn{1}{c}{Dist-1} &
  \multicolumn{1}{c}{Dist-2} &
  \multicolumn{1}{c}{RS-entail} &
  \multicolumn{1}{c}{Coherence} & \\
%  \multicolumn{1}{c}{Safety} \\
\hline
   \rowcolor{Gray}
\multicolumn{9}{l}{\textit{Baselines and Our Models}}
 \\
DialBart0-withguidelines     & 5.1   & 0.9   & 14.9  & 13.3 & 93.8 & 91.0 & 61.0 & 89.1 \\ % & 94.7 \\
OPT30B-fewshot       &  2.9  & 0.4	&12.0     & 10.1& 90.8&	91.4  & 27.5 &	71.0 \\ %&	93.1 \\
Bart-guideline-tuned           & 12.0  & 4.1   & 22.2  & {6.6}  & \textbf{93.3} & 93.0 & \textbf{89.4} & 88.5 \\ %& 95.0 \\
\dataname-tuned (Ours) & \textbf{12.4}  & \textbf{4.3}   & \textbf{23.0}  & \textbf{6.0} & 92.8 & \textbf{93.2} & 87.9 & \textbf{91.3} \\ %& 94.5 \\
Ref   responses           & 100.0 & 100.0 & 100.0 & 3.3  & 94.1 & 93.0 & 86.6 & 86.3 \\ %& 93.5\\
\hline 
 \rowcolor{Gray}
\multicolumn{9}{l}{\textit{Model Ablations for DialGuide model}}
 \\
BST-only         & 10.7  & 3.4   & 21.4  & 6.0  & 94.7 & 92.2 & 82.8 & 87.2 \\ %& 94.8 \\
No-guideline      & 6.0   & 1.2   & 16.2  & 1.2  & 92.3 & 93.4 & 34.0 & 91.1 \\ %& 94.5 \\
Multistep        & 5.5   & 1.1   & 15.6  & 2.5  & 92.3 & 92.7 & 81.6 & 87.9  \\ %& 94.9 \\
Ret-generate         & 5.7   & 2.4   & 16.4  & 2.2  & 90.2 & 90.4 & 84.5 & 83.9 \\ % & 94.6 \\
Ret-robust         & 7.0   & 1.7   & 17.0  & 3.1  & 92.9 & 93.0 & 79.0 & 86.9 \\ % & 94.8 \\
\bottomrule
\end{tabular}
\caption{Response generation results on \dataname-\textsc{BST} data. We compare our model \dataname-tuned with various zero-shot, few-shot and fine-tuned baselines.}
\label{tab:generationresults}
\vspace{-2mm}
\end{table*}


\subsection{Response Generation}
\subsubsection{Setup and Baselines}
This task involves generating a response $r$ that follows the provided guideline $g$ and is coherent to the dialogue context $C$.
We experiment on dev and test sets of \dataname-\textsc{BST} with 1438 and 1507 context-guideline-response triples. 
For training we experiment with both \dataname-\textsc{BST} and \dataname-\textsc{safety} train sets. Most of our baseline models are instruction-tuned, and we feed the following sequence as input to the models:  An instruction to generate a response, such as ``You will be shown a conversation between two people followed by a guideline for generating a response to the conversation. Generate a response that follows the guideline'', contatenated with the guideline and the dialogue context.
We consider the following baselines and models:
\begin{itemize}[noitemsep,nolistsep,leftmargin=*]
\item DialBart0-withguidelines: A Bart-large model pre-trained on Instructdial~\cite{gupta2022improving} tested on zero-shot generation with guidelines.
\item OPT30B-fewshot: An OPT~\cite{zhang2022opt} 30B model prompted using 3 in-context examples. 
\item Bart-guideline-tuned: A Bart-large~\cite{lewis-etal-2020-bart} model fine-tuned on our train set.
\item \dataname-tuned: A DialBart0 model fine-tuned on context-guideline-responses from our train set.
\item Ref-responses: The reference or gold responses from our \dataname-\textsc{BST} test set.
\item BST-only: A DialBart0 model fine-tuned only on \dataname-\textsc{BST} and not on \dataname-\textsc{safety}.
\item No-guideline: A DialBart0 tuned on conversations without conditioning on guidelines.
\item Multistep: A DialBart0-tuned model which  generates a guideline conditioned on the context (instead of using the provided guideline), then generates the response. 
% \item Dialbart-mixed: Model can generate based on both - guidelines or no guidelines
\item Ret-generate: A model that conditions on retrieved guidelines instead of gold guidelines during inference.
\item Ret-robust: The above model, but additionlly trained with noisy (randomly selected) guidelines for 20\% of the data. 
\end{itemize}


\subsubsection{Training and Evaluation Details}
We train all models using batch size 8 on 6 GPUs. The  models are provided with the dialogue context and the guideline as input and output the response as output.
The Ret-generate model is trained in the same manner as the \dataname-tuned model, but at inference time we retrieve the guidelines in two steps --- we first retrieve  a large set of guidelines using BM25 + DPR (100 from each) for faster inference, and then rerank these using the Rerank-Deberta (silver+ann) model from Section~\ref{sec:guidelineretrieval}. The final guideline  is selected randomly from the set of guidelines with a score greater than 98\% from the Deberta model.
The Ret-robust model is a variation of the Ret-generate model where the training data consists of additional instances with the gold guideline replaced with a random guideline for 20\% of the training data. This was done to make it more robust to incorrectly selected guidelines during inference.  

For evaluation we report Bleu-2,4 and RougeL scores based on reference responses. For diversity we report distinct-1,2. We measure the similarity between the guideline and the response using Bleu-2 and report it as Gd-Bleu-2. We use the response entailment model \greytext{BSTGuide} to measure whether the response follows the guideline and we name the metric RS-entail. Ideally a better model will have a high RS-entail and a low Gd-Bleu-2 score (response should avoid copying the guideline tokens). We measure coherence using a Bert-large model trained on a combination of conversations from the DEB dataset~\cite{sai-etal-2020-improving} and BST and Prosocial dialogue. This takes a pair of context and response as input and predicts if the response is coherent. 




% \begin{table*}[t]
% \small
% \centering
% \addtolength{\tabcolsep}{-1pt}
% % \setlength\tabcolsep{3pt}
% \begin{tabular}{lrrrrrrrrr}
% \toprule
% Model &
%   \multicolumn{1}{l}{Bleu-2} &
%   \multicolumn{1}{l}{Bleu-4} &
%   \multicolumn{1}{l}{RougeL} &
%   \multicolumn{1}{l}{Gd-Bleu-2} &
%   \multicolumn{1}{l}{Dist-1} &
%   \multicolumn{1}{l}{Dist-2} &
%   \multicolumn{1}{l}{RS-entail} &
%   \multicolumn{1}{l}{Coherence} &
%   \multicolumn{1}{l}{safety} \\
%   \midrule
% DialBart-rot                    & 8.9   & 2.1   & 18.2  & 14.2 & 89.3 & 94.4 & 93.5 & 92.0 & 99.7  \\
% % Dialbart-syntheticguidelines                    & 8.9   & 2.1   & 18.2  & 14.2 & 89.3 & 94.4 & 93.5 & 92.0 & 99.7  \\
% \dataname-tuned (Ours)  & 9.3   & 2.0   & 18.0  & 11.4 & 87.8 & 94.9 & 90.5 & 95.8 & 99.9  \\
% Ref-responses                 & 100.0 & 100.0 & 100.0 & 4.5  & 88.7 & 95.3 & 77.3 & 92.5 & 99.9 
% \\
% \hline 
%  \rowcolor{Gray}
% \multicolumn{10}{l}{\textit{Model Ablations (for DialBart)}}
%  \\
% No-guideline            & 7.3   & 0.7   & 15.9  & 3.6  & 82.2 & 95.3 & 47.0 & 96.3 & 99.7  \\
% % ret-generate, maybe multistep
% % Dialbart-ret-generate     &    &    &   &  &  &  &  &  &  \\
% Safety-only             & 9.5   & 2.1   & 18.8  & 11.6 & 88.3 & 94.9 & 88.5 & 95.0 & 100.0 \\
% BST-only         & 5.2   & 1.1   & 15.7  & 20.9 & 94.7 & 92.6 & 89.5 & 91.3 & 99.5  \\

% \bottomrule
% \end{tabular}
% \caption{Safety response generation results on \dataname-\textsc{safety} data.}
% \label{tab:safetygenerationresults}
% \vspace{-2mm}
% \end{table*}


% \begin{table}[t]
% \small
% \centering
% \addtolength{\tabcolsep}{-2pt}
% \setlength\tabcolsep{2pt}
% \begin{tabular}{lllll}
% \toprule
%     %   & \multicolumn{4}{c}{Human eval}                               \\
%     %  \hline
% Model & Coherence & Interest. & Specificity & Control  \\
% \hline
% DialBart0                 &  &  &  &  \\
% DialBart0-noguide                &  &  &  &  \\
% Bart-tuned                 &  &  &  &   \\
% DialBart0-tuned               &  &  &  &  \\
% Dialbart0-multistep    &  &  &  &   \\
% % Dialbart0-mixed    &  &  &  &  &  &  &  &  &   \\
% Dialbart0-ret-gen  &  &  &  &   \\
% Dialbart0-robust    &  &  &  &   \\
% \bottomrule
% \end{tabular}
% \caption{Response generation human evaluation}
% \label{tab:generationhumanresults}
% \vspace{-2mm}
% \end{table}


% \begin{table*}[t]
% \small
% \centering
% \addtolength{\tabcolsep}{-1pt}
% \setlength\tabcolsep{3pt}
% \begin{tabular}{llllll|llll}
% \toprule
%       & \multicolumn{5}{c}{Automatic metrics}         & \multicolumn{4}{c}{Human eval}                               \\
%      \hline
% Model & BLEU2 & Rouge & Distinct & DEB & Guideline-RS & Coherence & Interesting & Specificity & Control  \\
% \hline
% DialBart0                &  &  &  &  &  &  &  &  &  \\
% DialBart0-tunednoguide                &  &  &  &  &  &  &  &  &  \\
% Bart-tuned                &  &  &  &  &  &  &  &  &   \\
% DialBart0-tuned                &  &  &  &  &  &  &  &  &  \\
% Dialbart0-multistep    &  &  &  &  &  &  &  &  &   \\
% % Dialbart0-mixed    &  &  &  &  &  &  &  &  &   \\
% Dialbart0-retrieve-generate &  &  &  &  &  &  &  &  &   \\
% Dialbart0-tuned-robust    &  &  &  &  &  &  &  &  &   \\
% \bottomrule
% \end{tabular}
% \caption{Response generation results}
% \label{tab:generationresults}
% \vspace{-2mm}
% \end{table*}


% \begin{table*}[t]
% \small
% \centering
% \addtolength{\tabcolsep}{-1pt}
% \setlength\tabcolsep{3pt}
% \begin{tabular}{lllllll|lllll}
% \toprule
%       & \multicolumn{6}{c}{Automatic metrics}         & \multicolumn{5}{c}{Human eval}                               \\
%      \hline
% Model & BLEU2 & Rouge & Distinct & DEB & Guideline-RS & Safety & Coherence & Interesting & Specificity & Control & Safety \\
% \hline
% DialBart0                &  &  &  &  &  &  &  &  &  &  &  \\
% DialBart0-ROT                 &  &  &  &  &  &  &  &  &  &  &  \\
% DialBart0-generalsafety   &  &  &  &  &  &  &  &  &  &  &  \\
% DialBart0-generic-guide        &  &  &  &  &  &  &  &  &  &  &  \\
% DialBart0-safety         &  &  &  &  &  &  &  &  &  &  &  \\
% DialBart0-generic+safety &  &  &  &  &  &  &  &  &  & &  \\
% DialBart0-ret+generate &  &  &  &  &  &  &  &  &  & &  \\
% \bottomrule
% \end{tabular}
% \caption{Safety response generation results}
% \label{tab:safetyresults}
% \vspace{-2mm}
% \end{table*}


\begin{table*}[t]
\small
\centering
\addtolength{\tabcolsep}{-1pt}
\setlength\tabcolsep{3pt}
\begin{tabular}{lrrrrrrrrr}
\toprule
Model &
  \multicolumn{1}{l}{Bleu-2} &
  \multicolumn{1}{l}{Bleu-4} &
  \multicolumn{1}{l}{RougeL} &
  \multicolumn{1}{l}{Gd-Bleu-2 $\downarrow$} &
  \multicolumn{1}{l}{Dist-1} &
  \multicolumn{1}{l}{Dist-2} &
  \multicolumn{1}{l}{RS-entail} &
  \multicolumn{1}{l}{Coherence} &
  \multicolumn{1}{l}{Safety} \\
  \midrule
DialBart0-noguideline & 1.2 & 0.2 & 9.1 & 16.1 & 94.5 & 90.9 & 19.3 & 93.1 & 86.3\\
DialBart0-withguideline & 3.0 & 0.3 & 12.1 & 15.6 & 92.6 & 93.6 & 72.3 & 82.8 & 91.7\\
DialBart-rot     & 8.5   & 1.5   & 17.4  & 14.2 & 86.0 & 94.8 & 61.7 & 96.0 & 94.0  \\
OPT30B-fewshot   & 3.9   & 0.5   & 12.8  & 2.0 & 88.0 & 94.5 & 54.9 & 85.7 & 83.0  \\
% Dialbart-syntheticguidelines                    & 8.9   & 2.1   & 18.2  & 14.2 & 89.3 & 94.4 & 93.5 & 92.0 & 99.7  \\
\dataname-tuned (Ours)  & 8.3   & 1.5   & 17.2  & 11.4 & 88.0 & 95.2 & 96.3 & 95.3 & 92.4  \\
Ref-responses                 & 100.0 & 100.0 & 100.0 & 4.5  & 88.2 & 95.2 & 93.9 & 91.6 & 90.7 
\\
\hline 
 \rowcolor{Gray}
\multicolumn{10}{l}{\textit{Model Ablations for DialGuide model}}
 \\
No-guideline            & 7.3   & 1.0   & 16.1  & 3.6  & 85.4 & 95.4 & 47.0 & 94.9 & 92.6  \\
% ret-generate, maybe multistep
% Dialbart-ret-generate     &    &    &   &  &  &  &  &  &  \\
Safety-only             & 9.1   & 1.6   & 18.1  & 11.6 & 87.3 & 95.3 & 96.0 & 93.4 & 92.8 \\
BST-only         & 4.6   & 1.0   & 14.5  & 15.5 & 94.3 & 93.2 & 93.9 & 89.7 & 92.3  \\

\bottomrule
\end{tabular}
\caption{Safe response generation results on \dataname-\textsc{safety} data. We compare our model \dataname-tuned with various zero-shot, few-shot and fine-tuned baselines.}
\label{tab:safetygenerationresults}
\vspace{-2mm}
\end{table*}





\subsubsection{Results}
%JH: these seem more like notes than sentences -- is there more to add?
Table~\ref{tab:generationresults} presents results of automatic metrics for the \dataname-\textsc{BST} test set data.  The DialBart0-zeroshot model does not follow the guideline (low RS-entail) and copies guideline tokens (high Gd-Bleu-2).
The OPT30B-fewshot model which uses few-shot in-context examples is not able to match the performance of fine-tuned models. 
Since \dataname-tuned is pretrained on multiple dialogue tasks, it performs slightly better than its Bart-guideline-tuned version on most metrics, and is better at coherence.
\dataname-tuned (trained on both BST and safety datasets) performs better than BST-only, indicating that models can improve with more and more diverse data and guidelines.
Not conditioning on guidelines (the No-guideline model) does not effect coherence, but shows lower performance on other metrics. Additionally, our model provides the additional benefit of control over the generation space.
The Multistep model that  generates the guidelines and then generates the response  suffers slightly in quality;  however, it offers an end-to-end approach as well as interpretability to the model’s response generation. 
% While all baselines  use gold guidelines from our annotated data, DialBart-ret-generate generates a response based on a retrieved guideline.
The Ret-generate model that uses a retrieved guideline to generate the response has slightly lower performance, especially with diversity; however, its performance is still close to our best models. This shows that our \dataname framework can perform well with retrieved guidelines instead of gold guidelines.
The Ret-robust model that is trained to be robust to incorrectly retrieved guidelines performs better than the Ret-generate model on {coherence} and diversity metrics but is slightly poorer on {guideline entailment}. This shows that training a model by adding some noise can help the performance in a practical setting with retrieved guidelines.


\subsection{Dialogue Safety Experiments}
\subsubsection{Setup and Baselines}
This task involves generating a safe response $r$ based on a guideline $g$ that is coherent to the dialogue context $C$.
We experiment on the dev and test sets of \dataname-\textsc{safety} with 396 and 379 context-guidelines-response triples. The guidelines considered for testing in this experiment belong exclusively to the  \dataname-\textsc{safety} data.
% We train on data from \dataname-\textsc{safety} train sets. 
We consider the following baselines and models:
\begin{itemize}[noitemsep,nolistsep,leftmargin=*]
% \begin{itemize}
% \item DialBart0-zeroshot - Model trained on Instructdial which includes some safety related tasks.
\item DialBart0-noguideline:  A Bart-large model pre-trained on Instructdial~\cite{gupta2022improving} tested on zero-shot generation without guidelines.
\item DialBart0-withguideline:  A Bart-large model pre-trained on Instructdial~\cite{gupta2022improving} tested on zero-shot generation with guidelines.
\item DialBart-rot:  A Bart-large model pre-trained on Instructdial~\cite{gupta2022improving} tested on zero-shot generation with guidelines.
\item OPT30B-fewshot: An OPT 30B model prompted using 3 in-context examples. 
\item DialBart-rot: A DialBart0 tuned on RoTs~\cite{kim_prosocialdialog_2022} with comparable 
 count of instances.
\item \dataname-tuned (Ours): A Dialbart0 trained on a mixture of BST and safety guidelines data.
\item Ref-responses: The reference or gold responses from our \dataname-\textsc{safety} test set.
\item No-guideline: A Dialbart0 model tuned on safety data without guidelines.
\item BST-Only: A Dialbart0 trained on \dataname-\textsc{BST} dataset, without using safety data.
\item Safety-only: The Dialbart0 model trained on safety guideline data.
% \item DialBart0-ret-generate:  Model that conditions on retrieved guidelines instead of gold guidelines. 
\end{itemize}


In addition to the evaluation metrics used above for the generated responses, for the safety domain we include a Safety metric, which scores whether a response is safe. The safety classifier is a Deberta-large classifier trained on a  BAD (Bot Adversarial Dialogue) dataset~\cite{xu_bot-adversarial_2021} which consists of dialogue safety data and labels collected through an adversarial human-and-model-in-the-loop framework.
% \subsubsection{Training Details}

\subsubsection{Results}
We present the results in Table~\ref{tab:safetygenerationresults}. 
DialBart0-noguideline that performs zero-shot genertion on our test set without guideline performs poorly on safety. DialBart0-withguideline that conditions on guidelines in a zero-shot setting improves safety by 5\% points. 
OPT30B-fewshot model is able to generate guideline conditioned responses, but shows poor performance in terms of safety and coherence. 
The Dialbart-rot baseline  uses RoTs or rules of thumbs (such as ``it is bad to be racist''). ROTs do not contain the if condition (for example, “If someone wants to steal food”), and thus selecting the correct ROT at test time is more difficult than selecting a guideline, since they do not contain the information about the contexts the ROTs are relevant for.
Dialbart-rot has similar performance to \dataname-tuned, however RoTs are often very generic which leads to poor control as evident by the lower RS-entail score (61.7).

We perform ablation experiments with a few baselines.
The No-guidelines baseline that is not trained on safety data without guidelines or RoTs can generate safe responses, but lacks control, whereas \dataname-tuned can generate safe responses based on the developer's agenda. Although Safety-only baseline trained exclusively on \dataname-\textsc{safety} performs better than BST-only, the peformance of BST-only trained on \dataname-\textsc{BST} is close to its performance, which implies that a model that uses guidelines can perform well on cross-domain settings. 
% Although the more practical model, Dialbart-ret-generate, that generates responses based on retrieved guidelines shows a slightly lower safety score and coherence; however, it still shows reasonable performance.
% Overall, our model \dataname-tuned performs the best.


% \section{Qualitative and Error Analysis}
% \label{sec:analysis}

% \noindent
% \textbf{Guideline Retrieval}
% - Model trained with adversarial responses. 
% - Overpredicts generic guidelines

% \noindent
% \textbf{Response Selection}
% - Model struggles with more abstract guidelines
% - Suffers from some biases

% \noindent
% \textbf{Response Generation}
% - Model struggles with more abstract guidelines

